PyFR v2.0.3: Towards Industrial Adoption of Scale-Resolving Simulations

PyFR is an open-source cross-platform computational fluid dynamics framework based on the high-order Flux Reconstruction approach, specifically designed for undertaking high-accuracy scale-resolving simulations in the vicinity of complex engineering geometries. Since the initial release of PyFR v0.1.0 in 2013, a range of new capabilities have been added to the framework, with a view to enabling industrial adoption of the capability. This paper provides details of those enhancements as released in PyFR v2.0.3, explains efforts to grow an engaged developer and user community, and provides latest performance and scaling results on up to 1024 AMD Instinct MI250X accelerators of Frontier at ORNL (each with two GCDs), and up to 2048 NVIDIA GH200 GPUs on Alps at CSCS.

==> figs/tikz/temp.tex <==
% DO NOT DELETE, used for tikz caching

==> insitu.tex <==
\section{Insitu Visualisation}

==> outlook.tex <==
\section{Outlook}

The outlook going forwards for PyFR is positive.  Beyond additional plugins to aid in common post-processing tasks the following specific areas will be primary focus points for future development.

\paragraph{Implicit time stepping.}
Several well-known convergence acceleration techniques, including geometric multigrid and residual averaging, are currently not available in PyFR.  The absence of these technologies negatively impacts the performance of the implicit time steppers within PyFR.  This, in turn, places a restriction on Reynolds number and furthermore results in PyFR being somewhat sensitive to mesh quality.

\paragraph{Dynamic load balancing.}
Currently, all PyFR simulations must be partitioned statically in advance of running the simulation.  This can make it challenging to load balance a mixed-element simulation---especially at scale.  The solution for this is dynamic load balancing where elements can be automatically moved between partitions at run-time.  Such work will require substantial restructuring of several of the file formats and data structures used within PyFR.  An additional benefit of this work will be the possibility for nodes to be added and removed from a simulation while it is running.

\paragraph{Cache blocking for GPUs.}
Over the past five years the amount of shared last-level cache available on GPUs has increased dramatically.  Whereas a 2017 vintage NVIDIA V100 GPU only has  \qty[exponent-mode = fixed, fixed-exponent = 0]{6}{\mebi\byte} of L2 cache against ${\sim}7.8$ TFLOP/s of double precision compute, a 2023 vintage Intel data centre max GPU can have up to \qty[exponent-mode = fixed, fixed-exponent = 0]{408}{\mebi\byte} of L2 cache against ${\sim}52$ TFLOP/s of compute.  This large increase makes cache blocking a viable approach for improving GPU performance.

\paragraph{Overset.}
Many problems contain grids in relative motion.  A popular approach for handling this situation is to have multiple overlapping, or \emph{overset}, grids with the solution being interpolated between grids as required for the simulation.  Future versions of PyFR are expected to incorporate support for the parallel direct cut approach of Crabill et al. \cite{crabill2018parallel}.  It is expected that the successful deployment of this technique will rely heavily on the aforementioned support for dynamic load balancing.

==> tikz/temp.tex <==
% DO NOT DELETE, used for tikz caching

==> turbulence.tex <==
\section{Turbulence Injection}
